De Bruijn graphs and powers of $3/2$

In this paper we consider the set ${\mathbb Z}^{\pm\omega}_{6}$ of two-way infinite words $\xi$ over the alphabet $\{0,1,2,3,4,5\}$ with the integer left part $\lfloor\xi\rfloor$ and the fractional right part $\{\xi\}$ separated by a radix point. For such words, the operation of multiplication by integers and division by $6$ are defined as the column multiplication and division in base 6 numerical system. The paper develops a finite automata approach for analysis of sequences $\left (\left \lfloor \xi \left (\frac{3}{2} \right)^n \right \rfloor \right)_{n \in {\mathbb Z}}$ for the words $\xi \in {\mathbb Z}^{\pm \omega}_{6}$ that have some common properties with $Z$-numbers in Mahler's $3/2$-problem. Such sequence of $Z$-words written under each other with the same digit positions in the same column is an infinite $2$-dimensional word over the alphabet ${\mathbb Z}_6$. The automata representation of the columns in the integer part of $2$-dimensional $Z$-words has the nice structural properties of the de Bruijn graphs. This way provides some sufficient conditions for the emptiness of the set of $Z$-numbers. Our approach has been initially inspirated by the proposition 2.5 in [1] where authors applies cellular automata for analysis of $\left(\left\{\xi\left(\frac{3}{2}\right)^n\right\} \right)_{n\in{\mathbb Z}}$, $\xi\in{\mathbb R}$.

==> Btop.tex <==
\[
\begin{aligned}
\begin{bmatrix}
0&0\\
2&0\\
4&0\\
\hline
0&0\\
0&1\\
3&0\\
3&1
\end{bmatrix}
\begin{bmatrix}
0&1\\
2&1\\
4&1\\
\hline
0&1\\
0&2\\
3&1\\
3&2
\end{bmatrix}
\begin{bmatrix}
0&2\\
2&2\\
4&2\\
\hline
0&3\\
0&4\\
3&3\\
3&4
\end{bmatrix}
\begin{bmatrix}
0&3\\
2&3\\
4&3\\
\hline
0&4\\
0&5\\
3&4\\
3&5
\end{bmatrix}
\begin{bmatrix}
0&4\\
2&4\\
4&4\\
\hline
1&0\\
1&1\\
4&0\\
4&1
\end{bmatrix}
\begin{bmatrix}
0&5\\
2&5\\
4&5\\
\hline
1&1\\
1&2\\
4&1\\
4&2
\end{bmatrix}
\begin{bmatrix}
1&0\\
3&0\\
5&0\\
\hline
1&3\\
1&4\\
4&3\\
4&4
\end{bmatrix}
\begin{bmatrix}
1&1\\
3&1\\
5&1\\
\hline
1&4\\
1&5\\
4&4\\
4&5
\end{bmatrix}
\begin{bmatrix}
1&2\\
3&2\\
5&2\\
\hline
2&0\\
2&1\\
5&0\\
5&1
\end{bmatrix}
\begin{bmatrix}
1&3\\
3&3\\
5&3\\
\hline
2&1\\
2&2\\
5&1\\
5&2
\end{bmatrix}
\begin{bmatrix}
1&4\\
3&4\\
5&4\\
\hline
2&3\\
2&4\\
5&3\\
5&4
\end{bmatrix}
\begin{bmatrix}
1&5\\
3&5\\
5&5\\
\hline
2&4\\
2&5\\
5&4\\
5&5
\end{bmatrix}
\end{aligned}
\]


==> aBtop.tex <==
\[
\begin{aligned}
\begin{bmatrix}
0&0\\
2&2\\
4&4\\
\hline
0&0\\
0&1\\
3&0\\
3&1
\end{bmatrix}
\begin{bmatrix}
0&1\\
2&3\\
4&5\\
\hline
0&1\\
0&2\\
3&1\\
3&2
\end{bmatrix}
\begin{bmatrix}
0&2\\
2&4\\
4&0\\
\hline
0&3\\
1&4\\
3&3\\
4&4
\end{bmatrix}
\begin{bmatrix}
1&4\\
3&0\\
5&2\\
\hline
1&0\\
1&1\\
4&0\\
4&1
\end{bmatrix}
\begin{bmatrix}
1&5\\
3&1\\
5&3\\
\hline
1&1\\
2&2\\
4&1\\
5&2
\end{bmatrix}
\begin{bmatrix}
0&3\\
2&5\\
4&1\\
\hline
1&4\\
1&5\\
4&4\\
4&5
\end{bmatrix}
\begin{bmatrix}
1&0\\
3&2\\
5&4\\
\hline
2&3\\
2&4\\
5&3\\
5&4
\end{bmatrix}
\begin{bmatrix}
1&1\\
3&3\\
5&5\\
\hline
2&4\\
2&5\\
5&4\\
5&5
\end{bmatrix}
\end{aligned}
\]


==> gBbottom.tex <==
%gB уникальный снизу
\[
\begin{aligned}
\begin{bmatrix}
0&2\\
2&2\\
4&2\\
\hline
0&3\\
1&0\\
3&0\\
4&3
\end{bmatrix}
\begin{bmatrix}
0&3\\
2&3\\
4&3\\
\hline
0&5\\
3&2
\end{bmatrix}
\begin{bmatrix}
1&2\\
3&2\\
5&2\\
\hline
2&3\\
5&0
\end{bmatrix}
\begin{bmatrix}
1&3\\
3&3\\
5&3\\
\hline
1&2\\
2&5\\
4&5\\
5&2
\end{bmatrix}
\begin{bmatrix}
0&0\\
0&4\\
2&0\\
2&4\\
4&0\\
4&4\\
\hline
0&0\\
3&3
\end{bmatrix}
\begin{bmatrix}
0&0\\
1&4\\
2&0\\
3&4\\
4&0\\
5&4\\
\hline
1&3\\
4&0
\end{bmatrix}
\begin{bmatrix}
0&1\\
0&5\\
2&1\\
2&5\\
4&1\\
4&5\\
\hline
0&2\\
3&5
\end{bmatrix}
\begin{bmatrix}
0&1\\
1&5\\
2&1\\
3&5\\
4&1\\
5&5\\
\hline
1&5\\
4&2
\end{bmatrix}
\begin{bmatrix}
0&2\\
0&3\\
2&2\\
2&3\\
4&2\\
4&3\\
\hline
0&4\\
3&1
\end{bmatrix}
\begin{bmatrix}
0&2\\
1&3\\
2&2\\
3&3\\
4&2\\
5&3\\
\hline
1&1\\
4&4
\end{bmatrix}
\begin{bmatrix}
1&0\\
1&4\\
3&0\\
3&4\\
5&0\\
5&4\\
\hline
2&0\\
5&3
\end{bmatrix}
\begin{bmatrix}
1&1\\
1&5\\
3&1\\
3&5\\
5&1\\
5&5\\
\hline
2&2\\
5&5
\end{bmatrix}
\\ 
\begin{bmatrix}
1&2\\
1&3\\
3&2\\
3&3\\
5&2\\
5&3\\
\hline
2&4\\
5&1
\end{bmatrix}
\begin{bmatrix}
0&0\\
0&1\\
0&4\\
0&5\\
2&0\\
2&1\\
2&4\\
2&5\\
4&0\\
4&1\\
4&4\\
4&5\\
\hline
0&1\\
3&4
\end{bmatrix}
\begin{bmatrix}
0&0\\
0&1\\
1&4\\
1&5\\
2&0\\
2&1\\
3&4\\
3&5\\
4&0\\
4&1\\
5&4\\
5&5\\
\hline
1&4\\
4&1
\end{bmatrix}
\begin{bmatrix}
1&0\\
1&1\\
1&4\\
1&5\\
3&0\\
3&1\\
3&4\\
3&5\\
5&0\\
5&1\\
5&4\\
5&5\\
\hline
2&1\\
5&4
\end{bmatrix}
\end{aligned}
\]

